Targeted synthetic data generation for tabular data via hardness characterization

Data augmentation via synthetic data generation has been shown to be effective in improving model performance and robustness in the context of scarce or low-quality data. Using the data valuation framework to statistically identify beneficial and detrimental observations, we introduce a simple augmentation pipeline that generates only high-value training points based on hardness characterization, in a computationally efficient manner. We first empirically demonstrate via benchmarks on real data that Shapley-based data valuation methods perform comparably with learning-based methods in hardness characterization tasks, while offering significant computational advantages. Then, we show that synthetic data generators trained on the hardest points outperform non-targeted data augmentation on a number of tabular datasets. Our approach improves the quality of out-of-sample predictions and it is computationally more efficient compared to non-targeted methods.

==> sections/acknowledgements.tex <==
\subsubsection*{Acknowledgments}
Use unnumbered third level headings for the acknowledgments. All
acknowledgments, including those to funding agencies, go at the end of the paper.

==> sections/conclusion.tex <==
The proposed approach bridges the gap between existing hardness characterization methods \citep{hard_cat}, which track statistics of interest during training to identify hard data points, and game theoretic approaches to data valuation \citep[primarily Data Shapley, introduced in][]{data_shapley}. 
